Fine-grained Analysis of In-context Linear Estimation: Data, Architecture, and Beyond

Recent research has shown that Transformers with linear attention are capable of in-context learning (ICL) by implementing a linear estimator through gradient descent steps. However, the existing results on the optimization landscape apply under stylized settings where task and feature vectors are assumed to be IID and the attention weights are fully parameterized. In this work, we develop a stronger characterization of the optimization and generalization landscape of ICL through contributions on architectures, low-rank parameterization, and correlated designs: (1) We study the landscape of 1-layer linear attention and 1-layer H3, a state-space model. Under a suitable correlated design assumption, we prove that both implement 1-step preconditioned gradient descent. We show that thanks to its native convolution filters, H3 also has the advantage of implementing sample weighting and outperforming linear attention in suitable settings. (2) By studying correlated designs, we provide new risk bounds for retrieval augmented generation (RAG) and task-feature alignment which reveal how ICL sample complexity benefits from distributional alignment. (3) We derive the optimal risk for low-rank parameterized attention weights in terms of covariance spectrum. Through this, we also shed light on how LoRA can adapt to a new distribution by capturing the shift between task covariances. Experimental results corroborate our theoretical findings. Overall, this work explores the optimization and risk landscape of ICL in practically meaningful settings and contributes to a more thorough understanding of its mechanics.

==> app/add_notations.tex <==
\section{Auxiliary Notations}

==> app/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: \textbf{All the theoretical contributions claimed in the abstract and introduction along with the underlying data model are presented in Section~\ref{sec:setup} and Section~\ref{sec:main}.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: \textbf{This is a theoretical study which (similar to prior studies in the field) relies on a precise but simplified data model to draw quantitatively precise conclusions. All the assumptions on the data model are clearly stated in Section~\ref{sec:setup} and Section~\ref{sec:main}. We have also added a paragraph after the conclusion to specifically highlight various limitations of our work.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: \textbf{As discussed above, for all of our theoretical results and proofs we state the precise setup and assumptions in Section~\ref{sec:setup} and Section~\ref{sec:main}. Due to page limit, proofs are deferred to the supplemental material.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: \textbf{This is primarily a theoretical work where detailed synthetic experiments (on the same data model studied in our theoretical analysis) have been conducted to corroborate our theoretical findings. We provide sufficient details in Section~\ref{sec exp} for reproducing these experiments.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \textbf{As discussed above, this paper conducts small scale synthetic experiments to corroborate our theoretical findings. We have provided sufficient details to reproduce these experiments in Section~\ref{sec exp}. We would be happy to share relevant Jupyter notebooks if that is deemed helpful during the review process.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}  
    \item[] Justification: \textbf{All the relevant details for our small scale experiments are provided in Section~\ref{sec exp}.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \textbf{This work is a theoretical work studying the optimization landscape of linear attention/H3 under population risk. Then our goal of simulations is to find the optimal solution corresponding to the minimal risks. Therefore, we do not report the error bars and we have included the discussion in the experiment section.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \textbf{Our work only focuses on 1-layer attention/H3 model training with hidden dimension $21$ and maximal context length $<100$, which can be implemented easily.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} 
    \item[] Justification: \textbf{Yes, the authors confirm that the research conducted in the paper conform wiht the NeurIPS Code of Ethics.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: \textbf{In its current form, we don't see any specific negative impacts of our theoretical study. However, we have discussed potential broader impacts of the future extensions of this work, e.g., the ones tied to eliciting undesirable behavior of LLMs with in-context learning, while discussing the limitations of the work after the conclusion section.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: \textbf{The synthetic setup studied in the paper does not pose such risks.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{}
    \item[] Justification: \textbf{The paper does not rely on existing assets.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer:\answerNA{}
    \item[] Justification: \textbf{The paper does not release new assets such as code, data, or models.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: \textbf{The paper does not involve crowdsourcing nor research with human subjects.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: \textbf{The paper does not involve crowdsourcing nor research with human subjects.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sec/fig_low_rank.tex <==
\begin{figure}[!t]
\centering
\begin{subfigure}{0.325\linewidth}
    \includegraphics[height=0.75\linewidth]{figs/rank_d5.pdf}
\caption{Low-rank ($d=5$)}\label{fig:low rank d5}
\end{subfigure}
\begin{subfigure}{0.325\linewidth}    
    \includegraphics[height=.75\columnwidth]{figs/rank_d20.pdf}
\caption{Low-rank ($d=20$)}\label{fig:low rank d20}
\end{subfigure}
\begin{subfigure}{0.325\linewidth}    
    \includegraphics[height=.75\columnwidth]{figs/lora_d20.pdf}
\caption{LoRA ($d=20$)}\label{fig:lora}
\end{subfigure}
\caption{Low-rank and LoRA experiments. In Figs.~\ref{fig:low rank d5} and \ref{fig:low rank d20}, we train low-rank linear attention by setting $\WK,\WQ\in\R^{(d+1)\times r}$ where $r$ is the rank restriction and $\W:=\WK\WQ^\top$. In Fig.~\ref{fig:lora}, we first pretrain the model using isotropic linear data. Then train additional $r$-rank LoRA weights to adapt the model to solve new distributed data using low rank matrices. }
\label{fig:low rank}
\end{figure}

==> sec/fig_overview.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=1\linewidth]{figs/overview_fig2.pdf}
% \caption{We investigate the optimization landscape of in-context learning from the lens of architecture choice, the role of distributional alignment, and low-rank parameterization.}
% of feature or task vectors
\label{fig:main}
%\vspace{-7pt}
\end{figure}

==> sec/idea.tex <==


\section{Problem Setup}

\noindent\textbf{In-context linear estimation.} Let prompt be $\Z=[\z_1^\top~\dots~\z_n^\top]^\top \in \R^{n \times (d+1)}$ where we set $\z_i=[\x_i^\top~y_i]^\top \in \R^{d+1}$ and $\z_{n+1}=[\x_{n+1}~0] \in \R^{d+1}$. When clear from context, we drop the subscript $n+1$ and set $\z=\z_{n+1},\x=\x_{n+1}$. The linear attention layer estimates the label $y$ associated to $\x$ via $F(\Z)=\z^\top\W\Z^\top\Z\vb$. Here $\hat\bt=\W\Z^\top\Z\vb$ provides an estimate of the true task vector $\bt$. Given a distribution $\Z\sim\Dc$, we optimize the linear attention layer as follows:
\[ 
\vbs,\Ws=\arg\min_{\vb,\W}\E[(y-F(\Z))^2].
\]
Suppose $\W=\begin{bmatrix}\W&\boldsymbol{0}\\?&?\end{bmatrix}\in\R^{(d+1)\times (d+1)}$ and $\vb=\begin{bmatrix}\boldsymbol{0}\\v\end{bmatrix}\in\R^{d+1}$. Then $\Z\vb=v\y$ and 
\[ 
F(\Z)=\z^\top \W\Z^\top \Z\vb=v \x^\top \W \X^\top \y.
\]
$\W\gets v\W$, $F(\Z)= \x^\top \W \X^\top \y$.
\begin{align} 
\E[(y-F(\Z))^2]&=\E[(\x^\top\bt-\x^\top \W \X^\top \y)^2]\\
&=\E[\x^\top (\bt- \W \X^\top \y)^2]=\E[ (\bt- \W \X^\top \y)\bSi(\bt- \W \X^\top \y)^\top]\\
&=\E[ \tn{\bSb(\bt- \W \X^\top \y)}]
\end{align}
\begin{definition}[Independent Data Model] We assume $\y_i=\x_i^\top\bt+w_i$ where $(\x_i)_{i=1}^{n+1}\sim\Nn(0,\bSi),\bt\sim\Nn(0,\B),(w_i)_{i=1}^{n+1}\sim\Nn(0,\sigma^2)$ are all independent. 
\end{definition}
\red{For vanilla analysis that prove optimal estimator is 1-step GD, we might not need Gaussian distribution.}

The papers \url{https://arxiv.org/pdf/2307.03576} and \url{https://arxiv.org/pdf/2306.00297} are providing a fairly detailed analysis of the standard data model above (under some assumptions on $\bSi,\B$). 

\noindent\textbf{Simplified Attention Model.} Assume $\w_{12}=0$ (top right of key-query) and $\vb_1=0$ (top $d$ entries of value). Justification: For independent data model, these cross-terms results in odd moments of the entries of the task $\bt$ and features $\x_i$ (e.g.~$\x^\top\W\x_i\x_i^\top\vb$ which is third order) whereas the target label $\x^\top\bt$ requires even moment terms. The fourth order term $\x^\top\w_{12}y_i\x_i^\top\vb$ can only explain 1 out of $d$ degrees of freedom of $\bt$, thus not useful for prediction as $d$ grows. Specifically, the fourth order term can only estimate $\bt$ using the fixed $\w_{12}$ direction via $\hat\bt=\w_{12}y_i\x_i^\top\vb$, thus can only reduce the error by a factor of $1/d$ (whenever distribution of $\bt$ sweeps all directions like $\Nn(0,\Iden)$).

%For our settings (RAG, Task-Feature alignment), these results in asymptotically inconsistent estimation i.e.~they provide noisy estimates as $n\rightarrow\infty$ hurting the eventual accuracy. Dedicate a section (potentially in appendix) to discuss why this assumption is warranted.

\subsection{How to analyze this model?} 
For simplicity, suppose covariances are isotropic and no noise. After some algebra, the analysis essentially boils down to the following expectation $\E[\tn{\bt-\W\X^\top\y}^2]$ where $\y=\X\bt$. Thus, we wish to study $\min_{\W}\E[\tn{(\Iden-\W\X^\top\X)\bt}^2]$. This can be approached in more than one ways. An important trick is orthogonal decomposition: Namely, let us set $\btb=\bt/\tn{\bt}$, $\g=\X\btb\sim\Nn(0,1)$, $\Xb=\X-\X\btb\btb^\top$, and observe that $\g,\Xb$ are independent and $\X=\Xb+\g\btb^\top$. We can then write
\begin{align}
\X^\top\X\btb=(\Xb^\top+\btb\g^\top)\g=\tn{\g}^2\btb+\Xb^\top\g.
\end{align}
Since $\g,\Xb$ are independent and $\Xb$ is effectively a $n\times (d-1)$ standard normal, the right hand side is approximately distributed as $\Nn(n\btb,n\Iden_d)$. In other words, using $\tn{\bt}\approx\sqrt{d}$, for $\hb\sim\Nn(0,\Iden_d)$,
\[ 
\frac{1}{n}\X^\top\y\approx \bt+\sqrt{\frac{d}{n}}\hb
\] 
Thus, 
\begin{align}
\E[\tn{\bt-\frac{1}{n}\W\X^\top\y}^2]&\approx \E[\tn{(\Iden-\W)\bt}^2]+\E[\tn{\W\hb}^2]/n\\
&=\text{trace}((\Iden-\W)(\Iden-\W^\top)+\frac{d}{n}\W\W^\top)\\
&=\text{trace}(\Iden-\W-\W^\top+(1+\frac{d}{n})\W\W^\top).
\end{align}
Differentiating, the optimal $\W$ is given by $\Ws\approx\frac{n}{n+d}\Iden$.

\vspace{-5pt}
\subsubsection{Analysis outline for general covariance}
We can use the above strategy but we should whiten the covariances. \red{I believe the analysis below already generalizes the results of \url{https://arxiv.org/pdf/2307.03576} which assumes $\bSi=\B^{-1}$.} For instance, set $\X=\Xa\bSb$ where $\bSb=\sqrt{\bSi}$ and $\Xa$ is now $\Nn(0,1)$. Now set $\bta=\bSb\bt$ and $\btb=\bta/\tn{\bta}$. We have $\X\bt=\Xa\bSb\bt=\Xa\bta$ and set $\g=\Xa\btb\sim\Nn(0,\tn{\btb}^2\Iden)$. We similarly decompose 
\[ 
\Xa=\Xb+\g\btb^\top
\] 
where $\Xb,\g$ are independent. Set $\Sb=\bSb\B\bSb$. Noting $\E[\tn{\bt_0}^2]=\tr{\Sb}:=M$, we can then write
\[
\frac{1}{n}\X^\top\y=\frac{1}{n}\bSb\Xa^\top\Xa\bta\approx \bSb(\bt_0+\sqrt{\frac{M}{n}}\hb).
\]
The MSE error is given by (after accounting for $\x$'s covariance)
\[ 
\E[\tn{\bt_0-\frac{1}{n}\bSb\W\X^\top\y}^2]=\E[\tn{\bt_0-\bSb\W\bSb(\bt_0+\sqrt{\frac{M}{n}}\hb)}^2]
\] 
Now define the change-of-variable $\Wz=\bSb\W\bSb$. Recalling $M=\tr{\Sb}$, we can then write
\begin{align}
\E[\tn{\bt_0-\Wz(\bt_0+\sqrt{\frac{M}{n}}\hb)}^2]&=\E[\tn{(\Iden-\Wz)\bt_0}^2]+\frac{M}{n}\tr{\Wz\Wz^\top}\\
&=M-2\tr{\Wz\Sb}+\tr{\Wz\Sb\Wz}+\frac{M}{n}\tr{\Wz\Wz^\top}.\label{loss function}
\end{align}

Differentiating, we basically obtain % and setting $\Sb=\sqrt{\Sb}$
\[ 
\Sb=\Sb\Wz+\frac{M}{n}\Wz\implies \Iden=(\Iden+\frac{M}{n}\Sb^{-1})\Wz\implies \Wz=(\Iden+\frac{M}{n}\Sb^{-1})^{-1}.
\] 
This then yields $\Ws=(\bSi+\frac{M}{n}\B^{-1})^{-1}$. This solution strictly generalizes and recovers the Identity covariance model. Crucially, through this, we can likely figure out what LoRa does. This is because performance is controlled by the combined covariance matrix $\Sb=\bSb\B\bSb$.

\begin{lemma}[Optimizing Low-rank Attention Weights]\label{low rank attn} Suppose we use attention parameterization $\W_q,\W_k\in\R^{d\times r}$ which enforces $\text{rank}(\W)\leq r$. Consider the population objective \eqref{loss function} given by
\[ 
\Lc(\Wz)=\tr{\Sb}-2\tr{\Wz\Sb}+\tr{\Wz\Sb\Wz}+\frac{M}{n}\tr{\Wz\Wz^\top}.
\]
Denoting $\la_i$ to be the $i$'th largest eiganvalue of $\Sb$, we have that 
\[
\min_{\text{rank}(\Wz)\leq r}\Lc(\Wz)=\tr{\Sb}-\sum_{i=1}^r\frac{\la_i^2}{\la_i+M/n}.
\]
Noting $\tr{\Sb}=\sum_{i=1}^n\la_i$ and removing the rank constraint, this reduces to the standard optimal risk
\[ 
\min_{\Wz}\Lc(\Wz)=\sum_{i=1}^d\frac{1}{n/M+1/\la_i}.
\]
\end{lemma}
\begin{proof} 
Let us parameterize $\Wz=\Ub\La\Ub^\top$ where $\Ub\in\R^{d\times r}$ is the eigenvectors of $\Wz$. We will first treat $\Ub$ as fixed and optimize $\La\in\R^{r\times r}$. We will then optimize $\Ub$. Fixing $\Ub$ and setting $\Sbb=\Ub^\top\Sb\Ub$ and setting $\Lc'(\La)=\Lc(\Wz)-\tr{\Sb}$, we have that 
\begin{align}
\Lc'(\La)&=\tr{\Sbb\La^2}+\frac{M}{n}\tr{\La^2}-2\tr{\La\Sbb}.
\end{align}
Differentiating, we obtain $\La^*=(\Iden+\frac{M}{n}\Sbb^{-1})^{-1}$. Let $\s_i$ denote the eigenvalues of $\Sbb$. Plugging in this value, we obtain the optimal risk given by
\[ 
\Lc^*:=\Lc^*(\Ub)=-\sum_{i=1}^r s_i (1+\frac{M}{ns_i})^{-1}=-\sum_{i=1}^r\frac{ns_i}{M/s_i+n}.
\]
Now observe that, the right hand side is strictly decreasing function of the eigenvalues $s_i$ of $\Ub^\top\Sb\Ub$. Thus, to minimize $\Lc^*(\Ub)$, we need to maximize $\sum_{i=1}^r\frac{ns_i}{M/s_i+n}$. It follows from Cauchy's interlace theorem that $s_i\leq \la_i$ where $\la_i$ is the $i$th largest eigenvalue of $\Sb$ since $\Sbb$ is an orthogonal projection of $\Sb$ on $\Ub$. Consequently, we find the desired bound.
\end{proof}


\noindent\textbf{Impact of LoRA:} Based on the above Lemma \ref{low rank attn}, under jointly-diagonalizable new and old eigenvalues of $\Sb,\Sb^{old}$ $(\la_i)_{i=1}^d,(\la_i^{old})_{i=1}^d$; LoRA obtains top $r$ eigenvalue indices $\Ic$ maximizing the function $\texttt{gain}_i=\frac{1}{n/M+1/\la^{old}_i}-\frac{1}{n/M+1/\la_i}$. That means, LoRA's risk is given by
\[ 
\Lc(\W_{lora})=\min_{|\Ic|\leq r,\Ic\subset[d]}\sum_{i\in\Ic}\frac{1}{n/M+1/\la_i}+\sum_{i\not\in\Ic}\frac{1}{n/M+1/\la^{old}_i}
\]
Note that, this only provides a lower bound as we have to prove that the optimal LoRA-updated model $\W_{lora}$ is also jointly diagonalizable with covariances $\Sb,\Sb^{old}$, and $\W^{old}$.


\begin{comment}
and letting $s_i=\Sbb_{ii}$, we have that
\begin{align}
\Lc'(\La)&=\tr{\Sbb\La^2}+\frac{M}{n}\tr{\La^2}-2\tr{\La\Sbb}\\
&=\sum_{i=1}^r \la_i^2(\frac{M}{n}+s_i)-2\la_is_i.
\end{align}
Differentiating, we obtain $\la^*_i=(1+\frac{M}{ns_i})^{-1}=s_i(s_i+\frac{M}{n})^{-1}$. Next, let us study the risk which is given by plugging the optimal $\La^*$
\[ 
\Lc^*=-\sum_{i=1}^d s_i (1+\frac{M}{ns_i})^{-1}=-\sum_{i=1}^d\frac{ns_i}{M/s_i+n}.%-\sum_{i=1}^d\frac{ns_i^2}{M+ns_i}=
\]
\noindent\red{\textbf{Basic LoRa analysis:}} Assume that new and old covariances are jointly diagonalizable (e.g.~$\bSi_{old},\bSi_{new}$). Write the loss function \eqref{loss function} in terms of a sum over eigenvalues. Then determine which $r$ eigenvalues of the old distribution's $\W_{\text{old}}$ should be updated and matched to new optimal $\W_{new}$ by LoRa.

Exact LoRa objective is: Suppose $\Wz$ is fixed
\begin{align}
\Lc(\Lb)=M-2\tr{(\Wz+\Lb)\Sb}+\tr{(\Wz+\Lb)\Sb(\Wz+\Lb)}+\frac{M}{n}\tr{(\Wz+\Lb)(\Wz+\Lb)^\top}.\label{loss function}
\end{align}
If $\Lb$ was full rank, solution is $\Lb_\st=(\Iden+\frac{M}{n}\Sb^{-1})^{-1}-\Wz$.
\end{comment}


\subsubsection{Simplifying assumptions} 
Initially, we can benefit from following assumptions:
\begin{itemize}
\item For standard data model, the optimal attention model has the form $\W=\begin{bmatrix}\W'&0\\0&0\end{bmatrix}$ where $\W'\in\R^{d\times d}$. The choice of bottom row has no impact beacuse we set $\z=[\x~0]$ which zeroes it out. Setting top-right column to 0 suppresses the label-feature term of the form $y_i\x$. For standard data model, it can be shown that, these label-feature terms increase the test error and are undesirable, thus, optimal solution zeroes them out.
\item Similarly, optimal value matrix has the form $\vb=\begin{bmatrix}\vb'\\v\end{bmatrix}$ where $\vb'=0$. $\vb'\in\R^d$ picks up second-order features $\x_i\x_i^\top$ which are not useful for prediction. Thus, optimal solution zeroes them out and only $v$ remains.
\item We can assume $\W'$ is a symmetric matrix. Again this should be proven for all optimal solutions, but it may simplify notation/analysis.
\end{itemize}
\begin{comment}
\begin{proposition}[Optimal Linear Attention]
\end{proposition}
\begin{proof} Without losing generality, denote $\W'\gets \begin{bmatrix}\W~\w\\0~0\end{bmatrix}$ since $\z=[\x~0]$ and final row of $\W$ gets hit by zero. Also set $\vb'\gets \begin{bmatrix}\vb\\v\end{bmatrix}$. Observe that 
\begin{align}
\W'\Z^\top\Z\vb&=\W\X^\top\X\vb+v\W\X^\top\y +\w\y^\top \X\vb+v\w\y^\top\y.
%&=\W\X^\top\X\vb+v\W\X^\top\X\bt +\w\bt^\top\X^\top \X\vb+v\w\bt^\top\X^\top\X\bt\\
\end{align}
The prediction error (w.r.t.~noiseless label $y$ i.e.~$\sigma^2$ subtracted for noisy label) is given by 
\[ 
\Lc(\vb,\W,\w)=\E[(\x^\top(\bt-\W'\Z^\top\Z\vb'))^2]=\E[\tn{\bt-\W'\Z^\top\Z\vb'}^2],
\]
assuming $\bSi=\Iden$. We observe that optimal error is given by fitting the $v\W\X^\top\y $ term. Setting $\W\gets v\W$, we aim to control
%Let $\bth$ be the estimate of $\bt$. We have that 
\begin{align}
\Lc(\vb,\W,\w)&=\E[\tn{\bt-\W\X^\top\y}^2]=\E[\tn{(\Iden-\W\X^\top\X)\bt-\sigma\W\X^\top\z}^2]\\
&=\E[(\Iden-\W\X^\top\X)\B(\Iden-\W\X^\top\X)]+\sigma^2\E[\tn{\W\X^\top\z}^2].
\end{align} 
\end{proof}
\end{comment}
\subsection{Non-standard Data Models}

\noindent\textbf{Scenario 1: Retrieval-Augmented Generation.} In this model, we draw the query vector $\x$ and task vector $\bt$. We then draw data $(\x_i)_{i=1}^n$ to be used in-context according to the rule $\text{corr\_coef}(\x,\x_i)\geq \alpha>0$. An alternative simpler model is assuming $\x_i\sim\Nn(\alpha\x,(1-\alpha^2)\Iden)$ with $\x\sim\Nn(0,\Iden)$. All labels obey $\y_i=\x_i^\top \bt+w_i$. The \textbf{key takeaway} is leveraging aligned ICL data for better prediction along query.

\noindent\textbf{Proof strategy.} Start by decomposing $\X^\top\X=(\rho\X'+\alpha \onebb\x^T)^T(\rho\X'+\alpha \onebb\x^T)$ where $\rho=\sqrt{1-\alpha^2}$ and $\X'$ has i.i.d.~$\Nn(0,1)$ entries. Proceed by writing $\X^\top\X\bt$ which will provide terms in the form $\x\x^\top\bt$. Hitting this with $\x^\top$ from left will provide a useful $\x^\top\bt$ term which will help estimate $y$.

\vspace{10pt}
\noindent\textbf{Scenario 2: Task-Feature Alignment.} In this model, we first draw $\bt$ and then draw $\x_i\sim\Nn(\alpha\bt,\bSi)$. The \textbf{key takeaway} is leveraging the task-feature alignment for stronger estimation of the task vector.

\noindent\textbf{Proof strategy.} Start by decomposing $\X^\top\X=(\rho\X'+\alpha \onebb\bt^T)^T(\rho\X'+\alpha \onebb\bt^T)$ where $\rho=\sqrt{1-\alpha^2}$ and $\X'$ has i.i.d.~$\Nn(0,1)$ entries. Proceed by writing $\X^\top\X\bt$ which will provide useful terms along $\bt$ direction.

\vspace{10pt}
\noindent\textbf{Scenario 3: Distribution Shift with LoRa.} We train the model on $\Dc_1=(\bSi_1,\B_1)$ distribution to obtain $\W_1$. We are then given a new distribution $\Dc_2=(\bSi_2,\B_2)$. We adapt to $\Dc_2$ using LoRa on $\W_1$, that is, we ask for $\W_2$ such that $\text{rank}(\W_2-\W_1)\leq r$. The \textbf{key takeaway} is understanding how LoRa enables adaptation (e.g. we expect LoRa to update along the principal eigendirections of the difference between the two task distributions/covariances).

\vspace{10pt}
\noindent\textbf{Scenario 4: State-Space Models.} We consider the H3-like convolutional model. In its seq2seq form, the model is given by
\[ 
\text{SSM}(\Z) = ((\Z\W_1 \odot \Z\W_2) \ast \fb) \odot (\Z\W_3),
\] 
where $\fb\in\R^n$ is a 1-D convolution filter and $\W_{1,2,3}$ are weight matrices that correspond to K/V/Q of the attention layer, respectively. $\fb$ facilitates the aggregation of the key-value products. As explained in Section \ref{ssm blueprint}, this model can be used to perform one gradient step similar to linear attention. The \textbf{key takeaways} are
\begin{itemize}
\item Establishing the first result on the loss landscape of SSM-based ICL. Does the optimal SSM take gradient step?
\item Can SSM solve a distribution beyond linear attention?
\end{itemize}
To address the second question, our hypothesis is that SSM can leverage the convolutional filter $\fb$ to capture positional priors. Specifically, rather than vanilla gradient step $\bth=\frac{1}{n}\W\X^\top\y$, SSM can make the position-weighted update $\bth=\frac{1}{n}\W\X^\top(\fb\odot\y)=\frac{1}{n}\sum_{i=1}^n\W \fb_i\x_i y_i$. Here through $\fb$, we can weight the samples, in practice, we can do a recency weighting based on SSM e.g. setting $\fb_i=\rho^i$ for $i\geq 1$ corresponds to applying exponential smoothing along the context window during ICL.

\noindent\textbf{Dataset Model for SSM (temporal task shift).} Consider the following dataset where task distribution is shifting over time. Specifically draw $\bt\sim\Nn(0,\Iden)$ and draw $\bt_i$ IID such that $\bt_i\sim\Nn(\alpha_i\bt,(1-\alpha_i^2)\Iden)$. This way, at time $i$, task vector is $\alpha_i$-correlated to the task vector at time $n+1$. Set data $y_i=\x_i^\top\bt_i+w_i$. We wish to show that these correlations can be captured by the optimal convolution filter $\fb$ to obtain better estimation.

\subsection{In-context Linear Estimation with SSM}\label{ssm blueprint}
To implement 1 gradient step in-context, let us consider the following 1 layer SSM block \footnote{\noindent\emph{Remark:} This model is similar to H3 \url{https://arxiv.org/pdf/2212.14052.pdf}.}
\[
\text{SSM}(Z) = ((ZW_1 \odot ZW_2) \ast F) \odot (ZW_3).
\]
Blueprint for in-context learning:
\begin{enumerate} 
\item Get $X=[x_1 \dots x_L]^\top$ via $X=ZW_1$
\item Get labels $Y$ via $Y=ZW_2$.
\begin{itemize}
\item Here we can set $W_2$ to be a vector so that $Y\in\R^L$ is enforced to be a vector (to help the model grab labels).
\end{itemize}
\item Elementwise product $E=X \odot Y\in\R^{L\times d}$
\item Convolve $E \ast F$ where causal filter $F=[0~\texttt{all\_ones}]\in\R^L$ to obtain $\hat{\beta} = X^TY$.
\begin{itemize}
\item Note that, filter is shifted by 1 to ensure we use first $i-1$ samples to predict $y_i$.
\item I bet we can use a state-space model and population minima will still be the all\_ones filter. 
\end{itemize}
\item Elementwise $\hat{\beta} \odot x_{L+1}$ and then collapse with $\texttt{all\_ones}\in\R^d$ to get prediction $\hat y$. Here, we simply set $W_3=W_1$.
\end{enumerate}




==> sec/table_main.tex <==
\begin{table}
  \caption{\ankit{Add caption...}}
  \label{table:main}
  \centering
  \begin{tabular}{lcc}
    \toprule
    % &\multicolumn{}{c}{$\min_{\W}\Lc(\W):=$}                   \\
    % \cmidrule(r){1-3}
    % Linear model& i.i.d. & RAG\\
    % Task 
    % \midrule
    % \multirow{3}{*}{Linear model}
    & i.i.d.&RAG\\
    &$\Nc(0,\Iden),\Nc(0,\Iden)$&$\Nc(0,\Iden),\Nc(\alpha\x_{n+1},(1-\alpha^2)\Iden)$\\
    % &$\Nc(0,\Iden)$& $\Nc(\alpha\x_{n+1},(1-\alpha^2)\Iden)$ \\
    \midrule
    $\W^\st$ & $\frac{1}{n+d+1}\Iden$  & $\frac{1}{(\alpha^2d+1)n+d}\Iden$     \\
    % \midrule
    $\Lcs/d$     & $1-\frac{n}{n+d+1}$ & $1-\frac{(\alpha^2d+1-\alpha^2)n}{(\alpha^2d+1)n+d}$      \\
    \bottomrule
  \end{tabular}
\end{table}
